RaBit: Parametric Modeling of 3D Biped Cartoon Characters with a Topological-consistent Dataset

Assisting people in efficiently producing visually plausible 3D characters has always been a fundamental research topic in computer vision and computer graphics. Recent learning-based approaches have achieved unprecedented accuracy and efficiency in the area of 3D real human digitization. However, none of the prior works focus on modeling 3D biped cartoon characters, which are also in great demand in gaming and filming. In this paper, we introduce 3DBiCar, the first large-scale dataset of 3D biped cartoon characters, and RaBit, the corresponding parametric model. Our dataset contains 1,500 topologically consistent high-quality 3D textured models which are manually crafted by professional artists. Built upon the data, RaBit is thus designed with a SMPL-like linear blend shape model and a StyleGAN-based neural UV-texture generator, simultaneously expressing the shape, pose, and texture. To demonstrate the practicality of 3DBiCar and RaBit, various applications are conducted, including single-view reconstruction, sketch-based modeling, and 3D cartoon animation. For the single-view reconstruction setting, we find a straightforward global mapping from input images to the output UV-based texture maps tends to lose detailed appearances of some local parts (e.g., nose, ears). Thus, a part-sensitive texture reasoner is adopted to make all important local areas perceived. Experiments further demonstrate the effectiveness of our method both qualitatively and quantitatively. 3DBiCar and RaBit are available at gaplab.cuhk.edu.cn/projects/RaBit.

==> figure/fig_SMCL_process.tex <==
\begin{figure}[htbp]
\centering
\begin{subfigure}[b]{0.11\textwidth}
        \centering
        \includegraphics[width=0.9\textwidth]{image/SMCL_process/fig_pred1.pdf}
        \caption{$\bar{M_S}$}
\end{subfigure}
\hfill %\hspace{0mm}
\begin{subfigure}[b]{0.11\textwidth}
        \centering
        \includegraphics[width=0.9\textwidth]{image/SMCL_process/fig_pred2.pdf}
        \caption{$F_S(B)$}
\end{subfigure}
\hfill %\hspace{0mm}
\begin{subfigure}[b]{0.11\textwidth}
        \centering
        \includegraphics[width=0.9\textwidth]{image/SMCL_process/fig_pred3.pdf}
        \caption{$F_P(M_S,\Theta)$}
\end{subfigure}
\hfill %\hspace{0mm}
\begin{subfigure}[b]{0.11\textwidth}
        \centering
        \includegraphics[width=0.9\textwidth]{image/SMCL_process/fig_pred4.pdf}
        \caption{$F_T(M_P,T)$}
\end{subfigure}
\caption{\textit{\textbf{RaBit}.} (a) indicates the mean T-pose model $\bar{M}_{S}$. Given shape parameter $B$ for body, a specific T-pose biped character is next reconstructed as (b) shows. (c) demonstrates the posed model after applying pose parameter $\Theta$. Finally, a complete textured model (d) is obtained with texture parameter $T$.}
\label{fig_SMBL_process}
\end{figure}

==> figure/fig_dataset_landmark.tex <==
\begin{figure}[htb]
  \centering
  \includegraphics[width= .98 \linewidth]{image/fig_fixing.pdf}
  \caption{\textbf{Model checking by body landmarks.} %The model in the middle is the template model with segmented texture. We show the qualified examples (green border) and unqualified examples (red border) for some segmented annotations. The disqualification of the lower left subgraph is because the eyes' label is away from the eye socket, while the disqualification of the lower right subgraph is because the patch represents the elbow is not in the middle of the arm.
  Body landmarks are shown in this template model. Once a new model is finished, we will examine the semantic correspondence by comparing the body landmarks on the new model and the template. Green boxes on top demonstrate the qualified examples. The red box on the left corner is unqualified because this body landmark on the eyes is too large to delineate the eye socket. The other red box on the right corner with the elbow landmark far from the wrist is also unqualified.
  }
  \label{fig_fix}
\end{figure}

==> figure/fig_dataset_topology_anno.tex <==
\begin{figure}[htb]
  \centering
  \includegraphics[width=.98 \linewidth]{image/fig_dataset_topology_anno.png}
  \caption{Annotation for same topology checking. The model in the middle shows our annotated texture on our template model, showing the right place of these annotation. On both sides show some correct and wrong cases after transferring to other models.}
  
  %a图template 加annotation
  %b 图模型+眼部黑线不在眼眶 (应该明显展示出来)
  %c 图模型+身体标注偏离中线
  %d 图模型 正确标注，展示 眼部线条。
  %b, c, d 图模型不一样
  \label{fig_dataset_topology_anno}
\end{figure}

==> figure/fig_demo.tex <==
% \begin{figure}[t]
%   \centering
%   \includegraphics[width=.98 \linewidth]{image/ref_img.png}
%   \caption{A gallery of the 3D face models created by the novice users.}
%   \label{fig:gallery_user}
% \end{figure}

==> figure/fig_normalize.tex <==

\begin{figure}%[htbp]
    \centering
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{image/norm-01.pdf}
    \end{subfigure}
    \hfill %\hspace{0mm}
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{image/norm-shoulder-centric.pdf}
    \end{subfigure}
\caption{(a) Bounding box normalization. (b) Shoulder-centric normalization.}
\label{fig_normalize}
\end{figure}

==> figure/fig_pca.tex <==
\begin{figure}[htb]
  \centering
  \includegraphics[width=.49 \linewidth]{image/fig_pca.png}
  \caption{Texture map reconstruction from PCA.}
  \label{fig_pca}
\end{figure}

==> figure/fig_sample1d.tex <==
\begin{figure*}[htb]
  \centering
  \includegraphics[width= .98 \linewidth]{image/fig_sample_batch.pdf} %sample1d
  \caption{Axe Sampling: We sampled the first three axes of PCA of the whole-based model and every part of the part-based model(denote with '*'). The value is increased for every group of models, from left to right.}
  \label{fig_sample1d}
\end{figure*}

==> figure/fig_sample_rabit.tex <==
\begin{figure}[tbp]
  \centering
  \includegraphics[width=.90 \linewidth]{image/sample_rabit.pdf}
  \caption{\textbf{Sample of \textit{RaBit}}. \textbf{TBD}}
  \label{fig_sample_rabit}
\end{figure}

==> figure/fig_teaser.tex <==
\begin{figure*}[htb!]
  \centering
  \includegraphics[width=.98 \linewidth]{image/fig_teaser3.png}
  \caption{We present \textit{\textbf{3DBiCar}}, the first large-scale repository of 3D bipedal cartoon characters manually created by professional artists. It contains 1646 topologically consistent, textured and skinned 3D high-quality models, spanning 17 different species. To fully exploit the power of \textit{3DBiCar}, we propose \textit{SMCL}, a parametric model for mesh, pose and texture generation. With \textit{3DBiCar} and \textit{SMCL}, inferring 3D bipedal character models from a single image becomes possible.}
  \label{fig_teaser}
\end{figure*}

==> figure/fig_texture_decoder.tex <==
\begin{figure}[htb]
  \centering
  \includegraphics[width=.98 \linewidth]{image/fig_texture_decoder.png}
  \caption{Structure of texture decoder.}
  \label{fig_texture_decoder}
\end{figure}

==> figure/fig_texture_map_sample.tex <==
\begin{figure}[htb]
  \centering
  \includegraphics[width=.49 \linewidth]{image/fig_texture_map_sample.png}
  \caption{Sample same-topologic texture map.}
  \label{fig_texture_map}
\end{figure}

==> figure/fig_texture_para.tex <==
% \begin{figure*}[htb]
%   \centering
%   \includegraphics[width= .98\linewidth]{image/texture_para2.png}
%   \caption{Texture Parameterizing}
%   \label{fig_texture_para}
% \end{figure*}

% \begin{figure*}[htb]
%   \centering
%   \includegraphics[width=0.98 \linewidth]{image/texture_para2.png}
%   \caption{Texture Parameterizing-placeholder}
%   \label{fig_texture_para}
% \end{figure*}


==> figure/valify_partbased.tex <==
\begin{figure}[htbp]
  \centering
  \includegraphics[width=.98 \linewidth]{image/fig_valid.pdf} %pose aug
  \caption{The reconstruction error on whole mesh (blue line)  and head part (red line). The figure also indicates the error of the whole body and head when the (b) curve reaches the minimum value.
  (a) Reconstruction error on head on part-based model. (b) Reconstruction error on whole model on part-based model. (c) Reconstruction error on head on whole-based PCA.  (d) Reconstruction error on whole model on whole-based wPCA.}
  \label{fig_valid_result}
\end{figure}


\begin{table}[ht]
    \renewcommand{\arraystretch}{1.3}
    \centering
    \resizebox{\columnwidth}{!}{
        \begin{tabular}{c||c|c}
        % \hline 
        Method & whole error ($\times 10^{-3}$) $\downarrow$ & head error ($\times 10^{-3}$) $\downarrow$ \\
        \hline \hline 
        Whole$-$based PCA   & 3.8142          & 4.0407 \\
        Whole$-$based wPCA  & 3.9725          & 3.4410 \\
        Part$-$based$\#$    & 2.9756          & 4.4906 \\
        Part$-$based$*$     & \textbf{2.8003} & \textbf{3.4308}  
        %  \hline
        \end{tabular}
        %result is check!
    }
    \caption{Quantitative results of mesh reconstruction among different method. In whole-based wPCA, hypherparameter $w_r$ is set as 1.5 in our impletement. Part-based$\#$ means the result of distributing parameter space evenly among different parts. Part-based$*$ means the best result in multiple parameter space allocation. 
    } 
    \label{tab_valid_result}
\end{table}

==> paper/01_intro_backup.tex <==
\section{Introduction}
\label{sec:intro}

With the rapid development of digitization, creating high-quality 3D articulated characters is highly demanded in game platforms, film industries, and metaverse applications. However, even for expert artists, digitizing a character in 3D is still labor-intensive and time-consuming. How to assist people in producing visually plausible 3D content efficiently has always been a fundamental research topic in computer vision and computer graphics. It is thus essential for building a generalized character parameterization for 3D content creation.

A biped character parameterization is of crucial generalization direction. First, biped character control is one of the most basic research tasks in 3D animation~\cite{coros2010generalized, sok2007simulating, lee2010data}. Secondly, the biped model for posing and animation is indispensable for the most popular 3D studio tools, such as Blender, Maya, 3DS Max, \etc. Last but not least, current character parameterization has made a great effort on human digitalization~\cite{cheng2018parametric, robinette2002civilian, sela2015computational,han2017deepsketch2face,cai2021landmark,wu2018alive} from the real world but none of these works focuses on the fictitious biped cartoon character digitization, which is 
currently in great demand in the area of gaming, filming and virtualizing. Therefore, it is imperative to build a high-quality 3D biped cartoon character parametric model for generalized 3D character digitalization. 

To implement prevailing learning-based parameterization for fictitious biped characters, a comprehensive cartoon dataset with both topological-consistent geometry and corresponding texture is necessary. Advanced 3D sensing devices make capturing 3D data from the real world convenient and further prompt a growing number of 3D people repositories~\cite{anguelov2005scape, ionescu2013human3, SMPL:2015, pishchulin2017building, STAR:2020}. Thanks to those human datasets, it is already possible to infer nearly accurate 3D digital avatars from single-view images with the help of parametric models~\cite{SMPL:2015, SMPL-X:2019, STAR:2020} and data-driven techniques~\cite{bogo2016keep,kanazawa2018end,pavlakos2018learning,choutas2022accurate}. Recent deep neural networks~\cite{kanazawa2018end, kolotouros2019spin, SMPL-X:2019} have achieved excellence in the task of 3D human reconstruction, significantly increasing efficiency in modeling 3D human-related content. 

Still, constructing a 3D fictitious cartoon dataset simultaneously considering shape, pose, and texture is quite difficult. There are two challenges in collecting and building such a dataset. First, 3D cartoon characters available online are always topologically inconsistent and lack corresponding textures, thus hard to be utilized for many fundamental tasks, such as parametric modeling, pose retargeting, and texture synthesis. Meanwhile, collecting corresponding paired images or skinned skeletons of random shared 3D models is nearly impossible, hindering them from directly applying in single-view reconstruction or animation generation tasks. Second, diversified species, complex geometric shapes, and variegated texture styles of cartoon characters have brought additional challenges in building a 3D textured and skinned cartoon character dataset.

In the beginning, we address the scarcity of data by introducing \textit{3DBiCar}, the first large-scale publicly available 3D biped cartoon character dataset. Firstly, \textit{3DBiCar} spans a wide range of 3D biped cartoon digitalization sources with topological-consistent geometry. It contains 1646 high-diversified 2D biped cartoon character images, and corresponding high-quality 3D models with textures containing 17 species and 4 image styles. Secondly, all the 3D models in \textit{3DBiCar} are animation-ready and unified in topology. The artists were asked to craft 3D models using a pre-defined template with several landmarks and rig them with a consistent skeleton. It paves the way for learning a skinned parametric geometric model to serve several vital tasks in visual computing such as shape reconstruction, pose tracking and character animation. Thirdly, since all 3D meshes in \textit{3DBiCar} are topologically uniform, each model can be unwrapped into a unified UV map and manually painted by artists according to the paired image. 

Next, with \textit{3DBiCar}, a 3D cartoon character parametric model \textit{BiCar} is further proposed to model the 3D fictitious biped character encoding shape, pose, and texture at the same time for generalized character digitization. \textit{BiCar} is a statistical model for 3D cartoon character generation, which embeds shape, pose, and texture to a low-dimensional parametric space simultaneously. For shape and pose modeling, with pioneering human parameterization~\cite{SMPL:2015}, numerous methods~\cite{MANO:SIGGRAPHASIA:2017, SMPL-X:2019, STAR:2020} have been proposed to learn 3D human model representation from scan data, and these parametric models are widely used for digitizing humans from input images~\cite{kanazawa2018end, kolotouros2019spin, SMPL-X:2019}. However, straightly adapting these blendershape approaches to \textit{3DBiCar} fails to reconstruct high-fidelity models texture from low-dimension parameters due to the diversity and complexity texture of cartoon characters, especially their heads. We tackled this problem by introducing a non-linear generative model parameterization. Current texture modeling benefiting from deep representation learning advances, several works~\cite{bengio2013representation, kingma2013auto, karras2019style, karras2020analyzing} served well in embedding images to a low-dimension latent space. Inspired by image domain transfer methods~\cite{karras2020analyzing, wang2018pix2pixHD, karras2019style}, we encode texture into a latent parametric space and adopt a UV generator to parameterize texture.

Furthermore, we conduct comprehensive experiments to evaluate the capability of \textit{BiCar}. Specifically, to probe the potential of \textit{BiCar},  we implement exhaustive applications, including single-view cartoon character reconstruction, 3D cartoon model editing, sketch-based character modeling, and 3D cartoon animation. Qualitative results demonstrate the superb usability of our proposed parametric model \textit{BiCar}.

To summarize, our contribution can be listed as follows:
\begin{itemize}
    \item We propose the first 3D cartoon parametric model \textit{BiCar} for biped character digitizations. Our parameterization models the shape, pose, and texture of the 3D fictitious biped character simultaneously. Moreover, for texture parameterization, we adopt a novel UV generator to encode texture into the parametric space. 
    \item We introduce \textit{3DBiCar}, the first large-scale publicly available 3D biped cartoon character dataset. It spans a great range of 3D biped cartoon digitalization sources. Our data contains 1,646 high-diversified 2D biped cartoon character images and corresponding high-quality 3D models with topological-consistent geometry as well as detailed textures.
    \item We conduct various applications on \textit{BiCar} to demonstrate the promising potential of our biped cartoon parametric model in single-view cartoon character reconstruction, 3D cartoon model editing, sketch-based character modeling, and 3D cartoon animation.
\end{itemize}

%In the rest of the paper, we first review some related works in the domain of shape reconstruction and image synthesis in Sec.~\ref{sec:related_works}. Next, Sec.~\ref{sec:dataset} presents the procedure of constructing \textit{3DBiCar}, while the following Sec.~\ref{sec:algorithm} elaborates the backend algorithm for building \textit{SMCL}. In Sec.~\ref{sec:application}, we demonstrate several applications showcasing the potential of \textit{3DBiCar} and \textit{SMCL}. Finally, we make a conclusion and discussion on this work in Sec.~\ref{sec:conclusion}.



==> paper/03_dataset.tex <==
\section{Dataset}
\label{sec:dataset}
\input{figure/fig_dataset_gallery}
\input{figure/fig_table}

Recently, researchers have made significant progress in digitizing realistic and articulated human characters. It is already possible to generate relatively accurate 3D real humans from simple inputs, even a single-view image or sparse strokes. However, no existing works focused on the efficient generation of 3D biped cartoon characters, which a great demand in gaming and filming. Reconstructing a 3D biped cartoon character from simple inputs still be challenging, mainly due to the lack of data. In this work, we propose to fill this gap by introducing \textit{3DBiCar}, the first large-scale full-body 3D biped character data. We introduce \textit{3DBiCar} in detail in the following aspects.

% In this section, we present a new dataset, \textit{3DBiCar}, for 3D cartoon characters and elaborate the pipeline to build such dataset. \textit{3DBiCar} consists of 1646 image-model pairs of 17 species in 4 styles in total. 3D cartoon models are crafted by professional artists matching the shape, pose, and the texture from collected images. Drivable eyeballs are also available in our dataset. For brief dataset demonstration, please refer to Fig.~\ref{fig_dataset_gallery}.

It is worth noted that all the 3D models are of a uniform topological structure. Each model consists of 40776 vertices and 40760 faces. We create a T-pose template 3D model first and then require artists to move vertices only in case of any operations that may destroy topological properties. For example, changing the connecting relationship and deleting or adding points are unacceptable. We also delineate a group of annotations for artists to maintain the property of uniform topology. 


\subsection{Image Collection}

%At the beginning, about a thousand images are collected from free sources on the Internet and paid electronic documents from businessman. To facilitate the modeler to better model and a high quality of the dataset, we sift out quality pictures with the following rules, which are applied for later filtering as well.
Initially, we collect as many images with cartoon characters as possible. These images should cover common species of 3D cartoon characters.
%We also involve in searching images in specific domains and species to avoid extremely unbalance among species and domains.
%Unusual species (e.g., frog and robot) are also collected in \textit{3DBiCar} and considered as a challenging part. 
About a thousand images are collected from accessible sources on the Internet. Meanwhile, to cover a wide range of species and enrich the dataset, we purchase cartoon images in e-books. Finally, we select qualified images according to the following rules. Based on such criteria, we can build a fine-modeling and high-quality dataset:
\begin{enumerate}
\item The images shall be clear. Images with low resolution, abnormal brightness, or contrast are not acceptable.
\item The cartoon characters shall be complete and obvious. Specifically, the occluded or out-of-view part of the cartoon character's body should be trivial. The limbs are required to be visible as well.
\item The cartoon characters shall be humanoid. All models are initial as T-pose 3D models and share a uniform topology. % For example, poultry with feathered hands does not appear in our dataset. % reduce modeling difficulty
\item Images with similar cartoon characters shall be removed. Excessive characters of the same kind are avoided to balance data distribution. 
\end{enumerate}

 Finally, we select 1646 cartoon character images covering 17 species in 4 styles to construct a wide-applicable bipedal cartoon character dataset. Fig.~\ref{fig_datainfo} illustrates the detailed data distribution.

\subsection{Dataset Building}
\input{figure/fig_dataset_pipeline}
The construction of our dataset consists of three steps: template design, model building, and model checking. It is impossible to collect an available dataset from 3D models on the internet. These in-the-wild models vary in skeleton and mesh topology. Applying parameterization methods such as SMPL to these models results in a loss of detail. First, the template design in our pipeline ensures a uniform standard for biped models. This standard next serves our model building while still allowing the artists to construct diverse cartoon models. Finally, we apply the model checking to verify all the cartoon meshes. 

%% why we build model through 2D pictures and 
% 3D biped models on the internet are not unified in the skeleton and topology. If we treat the models with SMPL's method to generate models with the uniform topology, some characters' feature details will be lost. And, in previous method, the eyes are not separated from the body, leading to undriveable eyes. Moreover, Some models lack texture and source images, leading to trouble in single view reconstruction with texture when given images. Thus, we make a completed dataset \textit{3DBiCar} including texture, source images, and unified skeleton-topology standard. 

%The pipeline of dataset building is illustrated in Fig. \ref{fig_dataset_pipeline}.
%  There are two common pipelines to build a 3D model dataset in previous works. 

%  On one hand, in realistic face\cite{blanz1999morphable, le2017uhdb31, bagdanov2011florence, cosker2011facs, cao2013facewarehouse} or human\cite{robinette2002civilian, ionescu2013human3} reconstruction tasks, raw 3D data are usually acquired by large scanning instruments. Then, Researchers register the pre-defined template model with scanned data by optimization methods to obtain 3D human datasets with the same topology. However, scanning 3D cartoon characters is hardly possible, and the registry method is not suitable for cartoon models. This pipeline is not considered in our case. 

%  On the other hand, an intuitive idea is to manually construct a 3D model in the virtual world and fit a template T-Posed model on it following SMPL\cite{SMPL:2015}. However, such data processing leads to loss of detail and body parts comparing with previous pipelines such as tails and manes. Furthermore, the excessive model diversity in the dataset may lead to problems such as fitting difficulties or self-intersecting models. So this pipeline is also not suitable for data construction. In this case, we propose a new model building pipeline consisting of model crafting and model checking to deal with the difficulties in previous methods.


\subsubsection{Template Design}
\label{template}
Our approach starts with a well-designed predefined template human model for \textit{3DBiCar}. As Fig~\ref{fig_template_design} shows, we first design a template taking into accounts all possible body parts in cartoon characters. (a) illustrates the template mesh. We highlight specific body structure including horns, ears, nose and tail. Next, to make a standard for body parts alignment, we annotate specific patch of vertices as body landmarks. (b) demonstrates our body landmark annotations for rigging, skinning, and model checking. Finally, UV maps are built to construct a vivid cartoon model with texture. (c) shows the UV map of eyes and body. 

\textbf{Mesh Design.} Due to the complexity of body structures in different cartoon species, some specific parts of the template require a high resolution in one cartoon character's body. For example, the trunk of an elephant and the tail of a fox require higher resolution than other samples. Therefore, we reserve sufficient vertices and faces at specific positions on the template to maintain the uniform topological properties between all models and to meet resolution requirements for special structures demonstrated on Fig.~\ref{fig_template_design}(a). Our template model for the character body consists of 38726 vertices and 38724 faces. It is worth noticing that we also model two drivable eyeballs with 2050 vertices and 2046 faces. To sum up, our template mesh includes 40776 vertices and 40760 faces in total.
% predefine model



%\subsubsection{Skeleton generation}%We further supply our batch-auto-bone-rigging method to allow the model to pose. 
\textbf{Body landmarks.} Given a template model, the key to rigging is to determine all the joints in the template. Specifically, we adopt $K=23$ joints ($J\in \mathbb R^{K\times 3}$) for our cartoon models. A naive way is manually annotating all vertices nearby the predefined joints on the template model. Then annotations can be transferred to other models with the property of the uniform topology. However, this method failed on the joints with large deformation of vertices, for example, the tailbone joint when there is a long or large tail. We apply two strategies to counter this problem. First, we determine joints by two patches of vertices that are relatively stable during deformation. Second, we use centers of bounding boxes of marked vertices rather than averages to avoid joint offsets caused by the imbalanced vertices in patches. Based on the annotations of joints, we build our annotation landmark to guide crafting and inspection by adding additional feature lines and points to heads, including eye sockets, lips, nose, and ears. Since our template is a human model, we utilize human skinning weights to initialize our skinning weights. And then finetune by artists to prevent the model from self-intersecting or excessive deformation of specific poses. %The visualization of skinning weights is given in "Skinning" of Fig. \ref{fig_template_design} % skinning weights

 \textbf{UV Map.} Texture of eyes and body relies on corresponding UV Map. This mappping for model texture is considered in two levels. First, we use continuous body UV to maintain continuity between parts and minimize unexpected chromatic aberrations on the mesh at the margin of UV. Second, we also adjust the proportion of specific positions in the UV to avoid low UV clarity in some crucial parts. %UV

 %The visualization of skinning weights is given in "Skinning" of Fig. \ref{fig_template_design} % skinning weights.

\subsubsection{Model Building}
 To construct the model mesh, we considers both the cartoon charater on the given picture and counterpart animal in real life. The artist first bears the characteristic of animal in mind according to the species of models. Then by carefully observing the composition of different parts on the provided image, the artist adjusts the model from global to local through the standard, move, clay, and smoothing operations provided by \textbf{ZBrush}, a digital sculpting and painting software.  %The artist also uses the "symmetry method" in Z-Blush to keep the model symmetrical. 
According to body landmarks on mesh, the artists ensure the consistency of the semantic body parts by keeping the body landmarks in the proper position.  %mesh deform
% red comment: I think I should mention prior knowledge here. or we say common knowledge

To paint the model texture, the artists strictly maintain the correspondence to the image for visible parts, while the unseen texture is reasonably guessed with Occam's razor for invisible parts. Additionally, the artists densify the points to create high-resolution textures. 

To fit the pose of models, artists determine model pose in the open 3D graphics software \textbf{Blender}. The artists should set reasonable poses according to given images without self-intersection.  % texture and pose

% As for the texture of the painting, both correspondence and rational reference are required. For the visible parts, the modeler strictly maintains the correspondence to the image. While for the invisible parts, the texture is reasonably guessed using Occam's razor. Additionally, the modeler densifies the points to create high-resolution textures. 
% Each model will pose in the free open source 3D graphics and image software \textbf{Blender} according to the given image.  % texture and pose

\subsubsection{Model Checking}
%\input{figure/fig_dataset_topology_anno}
Even though multiple constraints are introduced to create a qualified model during model crafting, artifacts in crafted models still exist. We conduct the quality test on every model in the beginning. A model is next considered acceptable after  subjective check among a self-inspection team. Otherwise, artists should rework the model to fix flaws.

% The quality test requires that the models have a uniform topology, each should contain the same number of vertices, faces, and edges and the same connections, which is performed by a comprehensive script.
The quality test performed by a script verifies that the models are topology consistent. All models should contain the same number of vertices, faces, and edges and the same connections. 

For subjective check, the self-inspection team will judge the model in three aspects, including semantic correspondence on topology, prior knowledge, and similarity with the image:

First, correspondence on topology has a significant impact on rigging. We transfer the body landmarks to every model and check whether the annotations are still in the correct position. For instance, the body landmark on eyes should delineate the eye socket, and the body landmark of the elbow should remain in the middle of the shoulder and wrist label as Fig. \ref{fig_fix} shows.

Second, besides the 3D information on the image, prior knowledge is also considered to build models. To get a consensus on prior knowledge, the self-inspection team will judge the model from the characteristics of the species. For instance, the jawbone of foxes should be more protruding than cats. 

Third, the models' mesh, pose, and texture should be similar to the images. We urge that for visible parts, the models should be identical to images as possible, while for invisible parts, artists should infer the model rationally. 


==> paper/03_dataset_backup.tex <==
\section{Dataset}
\label{sec:dataset}

\input{figure/fig_dataset_gallery}
\input{figure/fig_table}
%In this section, we present a new dataset of 3D bipedal cartoon characters as well as its data production process. Our dataset consists of 1646 image-model pairs among 17 species in 4 domains. We employed 6 artists to craft 3D models to match the shape, pose, and texture of the cartoon characters with images from the Internet. Some instances of our datasets are already shown in Fig.~\ref{fig_dataset_gallery}.
In this section, we present a new dataset, \textit{3DBiCar}, for 3D cartoon characters and elaborate the pipeline to build such dataset. \textit{3DBiCar} consists of 1646 image-model pairs of 17 species in 4 styles in total. 3D cartoon models are crafted by professional artists matching the shape, pose, and the texture from collected images. Drivable eyeballs are also available in our dataset. For brief dataset demonstration, please refer to Fig.~\ref{fig_dataset_gallery}.

It is worth noted that all the 3D models are of a uniform topological structure. Each model consists of 40776 vertices and 40760 faces. We create a T-pose template 3D model first and then require artists to move vertices only in case of any operations that may destroy topological properties. For example, changing the connecting relationship and deleting or adding points are unacceptable. We also delineate a group of annotations for artists to maintain the property of uniform topology. 


\subsection{Image Collection}

%At the beginning, about a thousand images are collected from free sources on the Internet and paid electronic documents from businessman. To facilitate the modeler to better model and a high quality of the dataset, we sift out quality pictures with the following rules, which are applied for later filtering as well.
Initially, we collect as many images with cartoon characters as possible. These images should cover common species of 3D cartoon characters.
%We also involve in searching images in specific domains and species to avoid extremely unbalance among species and domains.
%Unusual species (e.g., frog and robot) are also collected in \textit{3DBiCar} and considered as a challenging part. 
About a thousand images are collected from accessible sources on the Internet. Meanwhile, to cover a wide range of species and enrich the dataset, we purchase cartoon images in e-books. Finally, we select qualified images according to the following rules. Based on such criteria, we can build a fine-modeling and high-quality dataset:
\begin{enumerate}
\item The images shall be clear. Images with low resolution, abnormal brightness, or contrast are not acceptable.
\item The cartoon characters shall be complete and obvious. Specifically, the occluded or out-of-view part of the cartoon character's body should be trivial. The limbs are required to be visible as well.
\item The cartoon characters shall be humanoid. All models are initial as T-pose 3D models and share a uniform topology. % For example, poultry with feathered hands does not appear in our dataset. % reduce modeling difficulty
\item Images with similar cartoon characters shall be removed. Excessive characters of the same kind are avoided to balance data distribution. 
\end{enumerate}

 Finally, we select 1646 cartoon character images covering 17 species in 4 styles to construct a wide-applicable bipedal cartoon character dataset. Fig.~\ref{fig_datainfo} illustrates the detailed data distribution.

\subsection{Dataset Building}
\input{figure/fig_dataset_pipeline}
The construction of our dataset consists of three steps: template design, model building, and model checking. It is impossible to collect an available dataset from 3D models on the internet. These in-the-wild models vary in skeleton and mesh topology. Applying parameterization methods such as SMPL to these models results in a loss of detail. First, the template design in our pipeline ensures a uniform standard for biped models. This standard next serves our model building while still allowing the artists to construct diverse cartoon models. Finally, we apply the model checking to verify all the cartoon meshes. 

%% why we build model through 2D pictures and 
% 3D biped models on the internet are not unified in the skeleton and topology. If we treat the models with SMPL's method to generate models with the uniform topology, some characters' feature details will be lost. And, in previous method, the eyes are not separated from the body, leading to undriveable eyes. Moreover, Some models lack texture and source images, leading to trouble in single view reconstruction with texture when given images. Thus, we make a completed dataset \textit{3DBiCar} including texture, source images, and unified skeleton-topology standard. 

%The pipeline of dataset building is illustrated in Fig. \ref{fig_dataset_pipeline}.
%  There are two common pipelines to build a 3D model dataset in previous works. 

%  On one hand, in realistic face\cite{blanz1999morphable, le2017uhdb31, bagdanov2011florence, cosker2011facs, cao2013facewarehouse} or human\cite{robinette2002civilian, ionescu2013human3} reconstruction tasks, raw 3D data are usually acquired by large scanning instruments. Then, Researchers register the pre-defined template model with scanned data by optimization methods to obtain 3D human datasets with the same topology. However, scanning 3D cartoon characters is hardly possible, and the registry method is not suitable for cartoon models. This pipeline is not considered in our case. 

%  On the other hand, an intuitive idea is to manually construct a 3D model in the virtual world and fit a template T-Posed model on it following SMPL\cite{SMPL:2015}. However, such data processing leads to loss of detail and body parts comparing with previous pipelines such as tails and manes. Furthermore, the excessive model diversity in the dataset may lead to problems such as fitting difficulties or self-intersecting models. So this pipeline is also not suitable for data construction. In this case, we propose a new model building pipeline consisting of model crafting and model checking to deal with the difficulties in previous methods.


\subsubsection{Template Design}
\label{template}
Our approach starts with a well-designed predefined template human model for \textit{3DBiCar}. As Fig~\ref{fig_template_design} shows, we first design a template taking into accounts all possible body parts in cartoon characters. (a) illustrates the template mesh. We highlight specific body structure including horns, ears, nose and tail. Next, to make a standard for body parts alignment, we annotate specific patch of vertices as body landmarks. (b) demonstrates our body landmark annotations for rigging, skinning, and model checking. Finally, UV maps are built to construct a vivid cartoon model with texture. (c) shows the UV map of eyes and body. 

\textbf{Mesh Design.} Due to the complexity of body structures in different cartoon species, some specific parts of the template require a high resolution in one cartoon character's body. For example, the trunk of an elephant and the tail of a fox require higher resolution than other samples. Therefore, we reserve sufficient vertices and faces at specific positions on the template to maintain the uniform topological properties between all models and to meet resolution requirements for special structures demonstrated on Fig.~\ref{fig_template_design}(a). Our template model for the character body consists of 38726 vertices and 38724 faces. It is worth noticing that we also model two drivable eyeballs with 2050 vertices and 2046 faces. To sum up, our template mesh includes 40776 vertices and 40760 faces in total.
% predefine model



%\subsubsection{Skeleton generation}%We further supply our batch-auto-bone-rigging method to allow the model to pose. 
\textbf{Body landmarks.} Given a template model, the key to rigging is to determine all the joints in the template. Specifically, we adopt $K=23$ joints ($J\in \mathbb R^{K\times 3}$) for our cartoon models. A naive way is manually annotating all vertices nearby the predefined joints on the template model. Then annotations can be transferred to other models with the property of the uniform topology. However, this method failed on the joints with large deformation of vertices, for example, the tailbone joint when there is a long or large tail. We apply two strategies to counter this problem. First, we determine joints by two patches of vertices that are relatively stable during deformation. Second, we use centers of bounding boxes of marked vertices rather than averages to avoid joint offsets caused by the imbalanced vertices in patches. Based on the annotations of joints, we build our annotation landmark to guide crafting and inspection by adding additional feature lines and points to heads, including eye sockets, lips, nose, and ears. Since our template is a human model, we utilize human skinning weights to initialize our skinning weights. And then finetune by artists to prevent the model from self-intersecting or excessive deformation of specific poses. %The visualization of skinning weights is given in "Skinning" of Fig. \ref{fig_template_design} % skinning weights

 \textbf{UV Map.} Texture of eyes and body relies on corresponding UV Map. This mappping for model texture is considered in two levels. First, we use continuous body UV to maintain continuity between parts and minimize unexpected chromatic aberrations on the mesh at the margin of UV. Second, we also adjust the proportion of specific positions in the UV to avoid low UV clarity in some crucial parts. %UV

 %The visualization of skinning weights is given in "Skinning" of Fig. \ref{fig_template_design} % skinning weights.

\subsubsection{Model Building}
 To construct the model mesh, we considers both the cartoon charater on the given picture and counterpart animal in real life. The artist first bears the characteristic of animal in mind according to the species of models. Then by carefully observing the composition of different parts on the provided image, the artist adjusts the model from global to local through the standard, move, clay, and smoothing operations provided by \textbf{ZBrush}, a digital sculpting and painting software.  %The artist also uses the "symmetry method" in Z-Blush to keep the model symmetrical. 
According to body landmarks on mesh, the artists ensure the consistency of the semantic body parts by keeping the body landmarks in the proper position.  %mesh deform
% red comment: I think I should mention prior knowledge here. or we say common knowledge

To paint the model texture, the artists strictly maintain the correspondence to the image for visible parts, while the unseen texture is reasonably guessed with Occam's razor for invisible parts. Additionally, the artists densify the points to create high-resolution textures. 

To fit the pose of models, artists determine model pose in the open 3D graphics software \textbf{Blender}. The artists should set reasonable poses according to given images without self-intersection.  % texture and pose

% As for the texture of the painting, both correspondence and rational reference are required. For the visible parts, the modeler strictly maintains the correspondence to the image. While for the invisible parts, the texture is reasonably guessed using Occam's razor. Additionally, the modeler densifies the points to create high-resolution textures. 
% Each model will pose in the free open source 3D graphics and image software \textbf{Blender} according to the given image.  % texture and pose

\subsubsection{Model Checking}
%\input{figure/fig_dataset_topology_anno}
Even though multiple constraints are introduced to create a qualified model during model crafting, artifacts in crafted models still exist. We conduct the quality test on every model in the beginning. A model is next considered acceptable after  subjective check among a self-inspection team. Otherwise, artists should rework the model to fix flaws.

% The quality test requires that the models have a uniform topology, each should contain the same number of vertices, faces, and edges and the same connections, which is performed by a comprehensive script.
The quality test performed by a script verifies that the models are topology consistent. All models should contain the same number of vertices, faces, and edges and the same connections. 

For subjective check, the self-inspection team will judge the model in three aspects, including semantic correspondence on topology, prior knowledge, and similarity with the image:

First, correspondence on topology has a significant impact on rigging. We transfer the body landmarks to every model and check whether the annotations are still in the correct position. For instance, the body landmark on eyes should delineate the eye socket, and the body landmark of the elbow should remain in the middle of the shoulder and wrist label as Fig. \ref{fig_fix} shows.

Second, besides the 3D information on the image, prior knowledge is also considered to build models. To get a consensus on prior knowledge, the self-inspection team will judge the model from the characteristics of the species. For instance, the jawbone of foxes should be more protruding than cats. 

Third, the models' mesh, pose, and texture should be similar to the images. We urge that for visible parts, the models should be identical to images as possible, while for invisible parts, artists should infer the model rationally. 


==> paper/06_experiment.tex <==
% \input{figure/fig_interpolation}
% \input{figure/fig_assemble}
\input{figure/fig_mesh_result}
\input{figure/fig_texture_result}

\section{Experiments}
\label{sec:experiment}
In this section, we conduct comprehensive experiments to demonstrate the capacity of \textit{SMCL} and \textit{3DBiCar}. In \ref{sec:experiment-sampleing}, we present the parameterization of \textit{SMCL} with different sampling methods. In \ref{sec:experiment-svr}, we elabrate the implementation detail and further demonstrate the qualitative and quantitative result of our single view reconstruction. 
%\subsection{Shape Morphing}




\input{figure/wild_result}

\subsection{Single View Reconstruction}
\label{sec:experiment-svr}


%In this section, we will show training details and quantitative and qualitative results of our method.

To obtain reconstruction networks for single view reconstruction. We split \textit{3DBiCar} into a training set (including 1532 models) and a testing set (including 114 models). In order to reduce domain shift during the evaluation, we keep the distribution of test samples as consistent with the distribution of 3DBiCar. % as possible.

%Even though we pay much effort into \textit{3DBiCar}, compared with other datasets, the train set is so limited that the neural network may not converge well. 

We next render synthetic images for each model and apply image augmentation such as color jitter for data augmentation. Moreover, we also make use of these sampling methods as Sec.~\ref{sec:experiment-sampleing} to generate synthetic model-image pairs. To minimize the impact of data imbalances, we resample the training set to maintain the balance between raw and synthetic data.

\textbf{Mesh Reconstruction.} In part-based \textit{SMCL}, we perform PCA on symmetric structures simultaneously (e.g., left and right hands) to reduce the size of parts from 6 to 4. To make fair comparision between whole-based and part-based linear models, we fix the dimension of $\Theta$ to 72 and $B$ to 200 (74 dimensions for head part and 42 for others).
%50 dimensions for every part of the part-based model). 
\input{table/table_mesh_result}

MAE errors of $\Theta$ and P-MPJPE are used in the pose parameter for evaluation. We also report the Projection error (P-Proj) between manual 2D annotation and 2D projections of models after alignment to verify the pose consistency between our results and given pictures. To evaluate shape reconstruction, we use reconstruction loss under T-pose (T-rec) as a model shape metric instead of using reconstruction directly because of the strong coupling between the pose-related metric and the reconstruction metric. Our quantitative result in Tab. \ref{tab_mesh_result} demonstrate that our part-based model outperformed the whole-based model in all metrics. We also visualize the results as shown in Fig.~\ref{fig_mesh_result}. The results of the whole-based model are acceptable, while the part-based models are closer to ground truth models.

\input{table/table_texture_result}

\textbf{Texture Reconstruction.} We choose the principal component analysis (PCA) method for comparison. In this method, PCA is first applied to reduce the dimension of UV, and then the neural network is used to fit the reduced vector. In PCA method and styleGAN method, the dimension of $T$ is fixed to be 512.

MSE, PSNR and FID are used for evaluation. As shown in Tab. \ref{tab_texutre_result}), the styleGAN method outperformed the PCA method in all three metrics. The qualitative result in Fig.~\ref{fig_texture_result} illustrates that the UV from the styleGAN method is sharper, less artifact, and closer to ground truth. 

\textbf{Result of wild image} To show both mesh reconstruction and texture reconstruction, we collect some images and generate textured posed models after extracting main character from images(Fig.~\ref{fig_wildresult}).


==> paper/application.tex <==
\input{figure/fig_pipeline}

\section{Single View Reconstruction}
\label{sec:svr}
%In this section, we do several experiments to show the capacity of our dataset. 
%\subsection{Shape Morphing}

% This application provides a baseline for single view reconstruction by a single general character image.
In this section, we propose a baseline for single view reconstruction based on \textit{SMCL} and \textit{3DBiCar}. We can generate realistic cartoon models from a single image with a 2D cartoon character, even for a simple watercolor painting from children. Our baseline of single review reconstruction is shown in Fig. \ref{reconstruction:pipeline}. We first extract the cartoon character from the paired image. Given this extracted character, the encoder will map this input to low-dimensional latent parameters with two CNNs and three MLPs. We use \textit{3DBiCar} as supervision to train these networks. Next, the latent codes containing shape, pose, and texture parameters will be utilized for \textit{SMCL} to build a vivid 3D cartoon character. Notice that our \textit{SMCL} also address the eyes modeling besides the shape, pose, and texture.

\subsection{Mesh Reconstruction}
% ? Many methods for single-view human reconstruction %have a strong understanding of rely on key points, which derives from mature upstream algorithms (e.g., dense human pose estimation) or massive datasets (e.g., COCO including more than two hundred thousand people).

%However, the extreme scarcity of datasets and diversification of styles make it difficult for the neural network to %understand fit key points. 


%Input images are first encode by Resnet50 and the output feature of Resnet is processed by two decoupled MLPs to produce parameters of shape and pose respectively. Posed textured models are generate with \textit{SMCL} and then supervised by ground truth model.

% The loss functions are as follows:
For mesh reconstruction, we first design following loss functions to optimize shape parameter $B$ and pose parameter $\Theta$:

\begin{equation}
    L_{para} = \|B_{pred}-B_{gt} \|_1 + \|\Theta_{pred} - \Theta_{gt}\|_1
\end{equation}
where L1 distance serves relatively robust supervision in our dataset with diverse samples.
%In our dataset, the number of instance is relatively small, and the diversity is large, so we use L1 loss for a more robust result.

Next, to ensure generated shape close to the ground truth model, $L_{shape}$ for shape supervision is introduced: 
\begin{equation}
    L_{shape} = \| F_P(\Theta_{gt}, B_{pred}) - F_P(\Theta_{gt}, B_{gt}) \|_2
\end{equation}
where the L2 distance between each vertex is counted in two models. $\Theta_{gt}$ is adopted to consentrate on the shape parameter $B$ and avoid mutual influence of $\Theta$. 

Following the similar idea, $L_pose$ is proposed to supervise pose parameter $B$ by minimizing the distance between joints: %Using $\Theta_{gt}$ and $B_{pred}$ to predict a model for loss calculation aims to prevent mutual influence and urge for a milder and more accurate backward propagation.
\begin{equation}
    L_{pose} = \| F_J(F_P(\Theta_{pred}, B_{gt})) - F_J(F_P(\Theta_{gt}, B_{gt})) \|_2
\end{equation}
where $F_J:\mathcal{R}^{N \times 3} \rightarrow \mathcal{R}^{J \times 3}$ is the function to extract the position of joints from the model. %(please refer to Sec. \ref{template}. Similar as $L_{pose}$, $\Theta_{pred}$ and $B_{gt}$ to predict a model for loss calculation.
Finally, the loss function for mesh reconstruction is the combination of aformentioned terms:

\begin{equation}
    L = L_{para} + \lambda_s L_{shape} + \lambda_p L_{pose}
\end{equation}
where $\lambda_s$ and $\lambda_p$ are 1 during experiments.

We find it hard to fit the parameters of eye with only a few features from limited images. Thus $ratio_{ed}$ and $ratio_{eR}$ are set to be the average value. This setting generates reasonable eye reconstruction with few artifacts.
%For eye reconstruction, the neural network is hard to extract such small features from images with limited data. Thus we set $ratio_{ed}$ and $ratio_{eR}$ as the average of those in the training set. With such operations, reasonable eyeballs can be generated without apparent artifacts.




\subsection{Texture Reconstruction}
%In Fig. \ref{reconstruction:pipeline}, shows our
% The input images is first encoded by Resnet50 and then processed by MLP (the structure is shown in Fig. \ref{reconstruction:pipeline}). 
To reconstruct the texture from a given image $x$, we need to fit an Encoder $E$ to get texture parameter with the generator $G$ in \textit{SMCL}. 

The loss function consists of two parts. The first part $L_{pw}$ denotes the pixel-wise L2 loss between generated UV with input image $x$ and ground truth $UV_{gt}$.
\begin{equation}
    L_{pw}= \|UV_{gt} - G(E(x)) \|_2
\end{equation}

% where $E(\cdot)$ denotes encoder, $G(\cdot)$ denotes texture generator of \textit{SMCL}, of which parameters are fixed during training encoder.
The second part follows LPIPS\cite{zhang2018unreasonable} to learn perceptual similarities.
\begin{equation}
    L_{\mathrm{LPIPS}} = \|F(x) - F(G(E(x))) \|_2
\end{equation}
where $F(\cdot)$ denotes the perceptual feature extractor. In the end, the loss function for texture reconstruction is as follows:

\begin{equation}
    L_{UV} = L_{pw} + \lambda L_{\mathrm{LPIPS}}
\end{equation}
where $\lambda$ is constant 1 in our experiments.

\iffalse
To support texture generation from a single image, we need an encoder.
Given an image as input, we need an encoder to find the corresponding latent code so that we can generate 
Although the model of styleGAN is powerful in generating texture maps, the input of styleGAN is a random latent code, which means it can only generate random texture maps. So, it is challenging to generate the specific texture map given the carton image in the wild. 


We use Resnet as the encoder. The loss function is as follows:

\begin{equation}
    L = L_{2}(x) + L_{LPIPS}(x)
\end{equation}
Similar to pixel2style2pixel, we use pixel-wise L2 loss for an overall robust result.
\begin{equation}
    L_{2}(x) = \|x - G(x) \|_2
\end{equation}
Where $G(\cdot)$ denotes the generated texture map by our decoder.

Then, we add the LPIPS loss to improve the result.
\begin{equation}
    L_{LPIPS}(x) = \|F(x) - F(G(x)) \|_2
\end{equation}
Where $F(\cdot)$ denotes the perceptual feature extractor.

We do not use the identity loss since there is a difference between our texture maps and faces.
\fi




==> rebuttal_figure/fig_badcase.tex <==
\begin{figure}[htb]
  \centering
  \includegraphics[width=1.\linewidth]{rebuttal_image/rebuttle_bad_case.pdf}
  \caption{Left:A case fails on mesh reconstruction.Right: A case fails on texture reconstruction.}
  \label{badcase}
\end{figure}

==> rebuttal_figure/fig_uv_style.tex <==
\begin{figure}[htb]
  \centering
  \includegraphics[width=1.\linewidth]{rebuttal_image/uv3.pdf}
  \caption{Left: UV layouts and textures. Right: Image styles.}
  \label{uv_style}
\end{figure}

==> supp_figure/fig_assemble.tex <==
\begin{figure}
     \centering
     \begin{subfigure}[b]{0.1\textwidth}
         \centering
         \includegraphics[width=\textwidth]{supp_image/part-aware-sample/fig_assemble1.pdf}
         \caption{Arms}
     \end{subfigure}
     \hfill\hspace{-4mm}
     \begin{subfigure}[b]{0.1\textwidth}
         \centering
         \includegraphics[width=\textwidth]{supp_image/part-aware-sample/fig_assemble2.pdf}
         \caption{Legs}
     \end{subfigure}
     \hfill\hspace{-4mm}
     \begin{subfigure}[b]{0.1\textwidth}
         \centering
         \includegraphics[width=\textwidth]{supp_image/part-aware-sample/fig_assemble3.pdf}
         \caption{Head}
     \end{subfigure}
     \hfill\hspace{-4mm}
     \begin{subfigure}[b]{0.1\textwidth}
         \centering
         \includegraphics[width=\textwidth]{supp_image/part-aware-sample/fig_assemble4.pdf}
         \caption{Body}
     \end{subfigure}
     \hfill\hspace{-4mm}
     \begin{subfigure}[b]{0.1\textwidth}
         \centering
         \includegraphics[width=\textwidth]{supp_image/part-aware-sample/fig_assemble5.pdf}
         \caption{Concat}
     \end{subfigure}
     \caption{\textbf{Part-aware Sample}. By concating embeddings representing differet parts from different model, we can sample a new model(e) which assemble parts (a-d) from different models. In column (e), yellow texture means the collision between two different parts.}
\end{figure}

==> table/table_dataset.tex <==
%\iffalse
\begin{table}[!t]
    \renewcommand{\arraystretch}{1.3}
    \centering
    \resizebox{\columnwidth}{!}{
        \begin{tabular}{|c|cccc|c|}
        \hline 
        \diagbox{Species}{Categories} & Hand Drawn & Picture Book & Computer Design &  Toy & Subtotal\\
        \hline \hline
        Human      & 23(1)        &  37(2)           & 84(6)     &  71(4)	&  215(13)  \\
        \hline
        Bear       & 11(1)        &  50(3)           & 60(4)     & 15(1)	&	136(9) \\
        \hline
        Mouse      & 4(1)         &  50(3)           & 46(4)     & 15(1)            &  115(9)  \\
        \hline
        Cat        & 32(2)        &  50(3)           & 18(2)      & 14(1)        &  114(8)  \\
        \hline
        Tiger &  33(2)    &  50(3)           & 10(2)      & 20(1)            &  113(8)  \\
        \hline
        Dog      &  3(1)          &  40(2)           & 53(3)     & 15(1)           &  111(7) \\
        \hline
        Rabbit   &  17(1)         &  39(2)           & 36(3)     & 16(1)            &  108(7)  \\
        \hline
        Monkey   &  10(1)         &  50(3)          & 36(3)     & 12(1)             &  108(8)  \\
        \hline
        Elephant   &  25(2)       &  50(3)          & 16(2)     & 15(1)             &  106(8)  \\
        \hline
        Pig   &  8(1)             &  41(2)          & 37(2)     & 11(1)           &  97(6)  \\
        \hline
        Fox   &  30(2)       &  50(3)          & 15(2)     & -            &  95(7)  \\
        \hline
        Hippo   &  11(1)   &  50(3)          & 29(2)     & -           &  90(6) \\
        \hline
        Cattle    &  10(1)  &  15(1)          & 37(2)     & 18(1)          &  80(5) \\
        \hline
        Deer    &   1(1) &   18(1)  &   33(4)  &   5(0)   &   57(6)  \\
        \hline
        Sheep    &  19(1)        &  11(1)          & 24(2)     & -           &  54(4)  \\
        \hline
        Horse   &  -      &  7(1)          & 23(0)     & 7(1)          &  37(2)  \\
        \hline
        Wolf    &   5(0)   &   -   &   5(1)   &   -   &   10(1)  \\
        \hline
        Frog    &  -          &  -           & 2(1)      & -          &  2(1)  \\
        \hline
        Robot    &  -         &  -           & 2(1)      & -         &   2(1)   \\
        \hline \hline
        Total    &  242(19)         &  608(36)         & 566(46)    & 234(15)          &  1650(116)  \\
        \hline
        \end{tabular}
    }
    \caption{1650 collected image distribution among species and domains. '-' denotes that we cannot find qualified image in this part. And the number in "()" denotes the number of test instances in specific classification.}
    \label{tab_stat_collect}
\end{table}
%\fi


\iffalse % original table
\begin{table}[!t]
    \renewcommand{\arraystretch}{1.3}
    \centering
    \resizebox{\columnwidth}{!}{
        \begin{tabular}{|c|cccc|c|}
        \hline 
        \diagbox{Species}{Categories} & Hand Drawn & Picture Book & Computer Design &  Toy & Subtotal\\
        \hline \hline
        Human      & 23        &  37           & 84     &  71	&  215  \\
        \hline
        Bear       & 11        &  50           & 60     & 15	&	136 \\
        \hline
        Mouse      & 4         &  50           & 46     & 15            &  115  \\
        \hline
        Cat        & 32        &  50           & 18      & 14        &  114  \\
        \hline
        Tiger &  33    &  50           & 10      & 20            &  113  \\
        \hline
        Dog      &  3          &  40           & 53     & 15           &  111  \\
        \hline
        Rabbit   &  17         &  39           & 36     & 16            &  108  \\
        \hline
        Monkey   &  10         &  50          & 36     & 12             &  108  \\
        \hline
        Elephant   &  25       &  50          & 16     & 15             &  106  \\
        \hline
        Fox   &  30       &  50          & 15     & -            &  95  \\
        \hline
        Wolf    &   5   &   -   &   5   &   -   &   10  \\
        \hline
        Pig   &  8             &  41          & 37     & 11           &  97  \\
        \hline
        Horse   &  -      &  7          & 23     & 7          &  37  \\
        \hline
        Deer    &   1   &   18  &   33  &   5   &   57  \\
        \hline
        Hippo   &  11          &  50          & 29     & -           &  90 \\
        \hline
        Cattle    &  10        &  15          & 37     & 18          &  80 \\
        \hline
        Sheep    &  19        &  11          & 24     & -           &  54  \\
        \hline
        Frog    &  -          &  -           & 2      & -          &  2  \\
        \hline
        Robot    &  -         &  -           & 2      & -         &   2   \\
        \hline \hline
        Total    &  242         &  608         & 566    & 234          &  1650  \\
        \hline
        \end{tabular}
    }
    \caption{1650 collected image distribution among species and domains. '-' denotes that we cannot find qualified image in this part.}
    \label{tab_stat_collect}
\end{table}
\fi
